Controlling Pre-trained Language Models for Grade-Specific Text Simplification

Text simplification (TS) systems rewrite text to make it more readable while preserving its content. However, what makes a text easy to read depends on the intended readers. Recent work has shown that pre-trained language models can simplify text using a wealth of techniques to control output simplicity, ranging from specifying only the desired reading grade level, to directly specifying low-level edit operations. Yet it remains unclear how to set these control parameters in practice. Existing approaches set them at the corpus level, disregarding the complexity of individual inputs and considering only one level of output complexity. In this work, we conduct an empirical study to understand how different control mechanisms impact the adequacy and simplicity of text simplification systems. Based on these insights, we introduce a simple method that predicts the edit operations required for simplifying a text for a specific grade level on an instance-per-instance basis. This approach improves the quality of the simplified outputs over corpus-level search-based heuristics.

==> tables/edit_ops.tex <==
\begin{table}[t]
\centering
 \def\arraystretch{1.2}
 \setlength\tabcolsep{2.5pt}
\scalebox{0.75}{
\begin{tabular}{lcc}
 \toprule
  \textsc{\textbf{Metric}}  &  \textsc{\textbf{Grade Tokens}}  &  \textsc{\textbf{CP-Multi}} \\
\midrule
Splitting & 1.13 & 1.38 \\
Lexical Complexity & 8.30 & 8.22 \\
Levenshtein Similarity &  0.91 & 0.80\\
  \bottomrule
 \end{tabular}
 }
\caption{Quality Estimation Metrics on Newsela  dataset} \label{tab:newsela-quality}
% 
% \vspace{-0.8cm}
\end{table}



==> tables/outputs.tex <==

\begin{table*}[tbh]
\centering
\scalebox{0.85}{
\begin{tabular}{lp{13cm}}
      \rowcolor{gray!24}
         \textbf{\textsc{Model}} & \textbf{\textsc{Text}} \\

  \textsc{source (grade 12)} & {\fontfamily{cmss}\selectfont Paracho, the "guitar capital of Mexico," makes nearly 1 million classical guitars a year, many exported to the United States.}  \\
    \addlinespace[0.2cm]
    \textsc{reference (grade 5)} & \texttt{W\_1.19 C\_1.20 L\_0.89 WR\_0.98 DTD\_1.50   } \\
    & {\fontfamily{cmss}\selectfont Paracho is known as the "guitar capital of Mexico." The town makes nearly 1 million classical guitars a year, with many exported to the United States.}  \\
    \textsc{avg-grade} & \texttt{W\_0.95 C\_0.92 L\_0.72 WR\_0.96 DTD\_0.86 } \quad \quad SARI: 49.35\\
    & {\fontfamily{cmss}\selectfont Paracho is the capital of Mexico. It makes nearly 1 million classical guitars a year. Many of them are sold in the United States.} \\
    \textsc{cp-multi} & \texttt{W\_1.06 C\_1.04 L\_0.77 WR\_0.97 DTD\_1.06  }  \quad \quad SARI: 55.31 \\
    & {\fontfamily{cmss}\selectfont Paracho is the capital of Mexico. It makes nearly 1 million classical guitars a year. Many of them are exported to the United States.	} \\

       \midrule

  \textsc{source (grade 12)} & {\fontfamily{cmss}\selectfont Development of Hyperion, which took about 2 1/2 years, was jump-started by an idea from software engineer Brent Burley.}  \\
    \addlinespace[0.2cm]
    \textsc{reference (grade 5)} & \texttt{W\_0.96 C\_0.88 L\_0.68 WR\_1.09 DTD\_1.00   } \\
    & {\fontfamily{cmss}\selectfont It took about 2 1/2 years to develop Hyperion. It began with an idea from software engineer Brent Burley.}  \\
    \textsc{avg-grade} & \texttt{W\_0.95 C\_0.92 L\_0.72 WR\_0.96 DTD\_0.86 } \quad \quad SARI: 52.01\\
    & {\fontfamily{cmss}\selectfont Development of Hyperion took about 2 1/2 years. It was started by an idea from a software engineer named Brent Burley.	} \\
    \textsc{cp-multi} & \texttt{W\_1.08 C\_1.05 L\_0.73 WR\_1.06 DTD\_0.89 } \quad \quad SARI: 67.97 \\
    & {\fontfamily{cmss}\selectfont Development of Hyperion was jump-started by an idea from software engineer Brent Burley. It took about 2 1/2 years to develop.} \\

 \midrule

 \textsc{source (grade 12)} & {\fontfamily{cmss}\selectfont Back at the Chimpanzee Sanctuary Northwest, Foxie has six companions, all of whom were used for hepatitis experiments.}  \\
    \addlinespace[0.2cm]
    \textsc{reference (grade 5)} & \texttt{W\_1.19 C\_1.20 L\_0.89 WR\_0.98 DTD\_1.50} \\
    & {\fontfamily{cmss}\selectfont Back at the Chimpanzee Sanctuary Northwest, Foxie has six companions. They were also used for experiments. }  \\
    \textsc{avg-grade} & \texttt{W\_0.95 C\_0.92 L\_0.72 WR\_0.96 DTD\_0.86 } \quad \quad SARI: 52.05\\
    & {\fontfamily{cmss}\selectfont Foxie has six companions at the Chimpanzee Sanctuary Northwest. All of them were used for experiments.} \\
    \textsc{cp-multi} & \texttt{W\_1.12 C\_1.07 L\_0.74 WR\_0.94 DTD\_0.97   }  \quad \quad SARI: 49.91 \\
    & {\fontfamily{cmss}\selectfont Foxie lives at the Chimpanzee Sanctuary Northwest in Washington, D.C. He has six companions. All of them were used for experiments.	} \\

      

    
\bottomrule

\end{tabular}
}
\caption{Sample outputs using different control types.} 
\label{tab:output_example}
\end{table*}


% Grade 8, 5
% \begin{table*}[tbh]
% \centering
% \scalebox{0.85}{
% \begin{tabular}{lp{13cm}}
%       \rowcolor{gray!24}
%          \textbf{\textsc{Model}} & \textbf{\textsc{Text}} \\

%   \textsc{source (grade 8)} & {\fontfamily{cmss}\selectfont The two women fell seriously ill with tuberculosis. All three were taken by helicopter to a nearby city, where Jakarewãja and Amakaria spent months in a straw hut built on the grounds of a hospital.}  \\
%     \addlinespace[0.2cm]
%     \textsc{reference (grade 5)} & \texttt{W\_1.18 C\_1.16 L\_0.87 WR\_1.02 DTD\_0.64 } \\
%     & {\fontfamily{cmss}\selectfont The two women fell seriously ill with tuberculosis, a disease that can attack the lungs. All three were taken by helicopter to a nearby city. Jakarewãja and Amakaria spent months there in a straw hut on the grounds of a hospital.} \\
%     \textsc{grade-control} & \texttt{SG\_8 TG\_5} \\
%     & {\fontfamily{cmss}\selectfont The two women fell seriously ill. All three were taken by helicopter to a nearby city. Jakarewja and Amakaria spent months in a straw hut built on the grounds of a hospital.}  \\
%     \textsc{avg-grade} & \texttt{W\_0.95 C\_0.92 L\_0.76 WR\_0.97 DTD\_0.90}\\
%     & {\fontfamily{cmss}\selectfont The two women fell seriously ill with tuberculosis. Jakarewja and Amakaria spent months in a straw hut built on the grounds of a hospital. All three were taken by helicopter to a nearby city.} \\
%     \textsc{cp-multi} & \texttt{W\_0.98 C\_0.94 L\_0.74 WR\_0.97 DTD\_0.67} \\
%     & {\fontfamily{cmss}\selectfont The two women fell seriously ill with tuberculosis. Jakarewja and Amakaria spent months in a straw hut built on the grounds of a hospital. All three were taken by helicopter to a nearby city.} \\

%        \midrule

%   \textsc{source (grade 8)} & {\fontfamily{cmss}\selectfont The great American soul singer Aretha Franklin died Thursday, August 16 at the age of 76, her representative has said. She was reported to have been gravely ill with her family at her bedside.}  \\
%     \addlinespace[0.2cm]
%     \textsc{reference (grade 5)} & \texttt{W\_0.84 C\_0.80 L\_0.76 WR\_1.00 DTD\_0.80  } \\
%     & {\fontfamily{cmss}\selectfont The great American soul singer Aretha Franklin died Thursday, August 16. She was 76 years old. The singer was very ill and her family was at her bedside.} \\
%     \textsc{grade-control} & \texttt{SG\_8 TG\_5} \\
%     & {\fontfamily{cmss}\selectfont The great American soul singer Aretha Franklin died Thursday, August 16 at the age of 76, her representative has said. She was reported to have been gravely ill with her family at her bedside.}  \\
%     \textsc{avg-grade} & \texttt{W\_0.95 C\_0.92 L\_0.76 WR\_0.97 DTD\_0.90}\\
%     & {\fontfamily{cmss}\selectfont The great American soul singer Aretha Franklin died Thursday, August 16 at the age of 76. She had been very ill with her family at her bedside. Franklin was 76 years old.} \\
%     \textsc{cp-multi} & \texttt{W\_0.97 C\_0.95 L\_0.77 WR\_0.98 DTD\_1.00} \\
%     & {\fontfamily{cmss}\selectfont The great American soul singer Aretha Franklin died Thursday, August 16 at the age of 76. She was reported to have been ill with her family at her bedside. Franklin was 76 years old.} \\
    
% \bottomrule

% \end{tabular}
% }
% \caption{Sample outputs using different control types.} 
% \label{tab:output_example}
% \end{table*}

